A Vision for Flexibile GLSP-based Web Modeling Tools

In the past decade, the modeling community has produced many feature-rich modeling editors and tool prototypes not only for modeling standards but particularly also for many domain-specific languages. More recently, however, web-based modeling tools have started to become increasingly popular for visualizing and editing models adhering to such languages in the industry. This new generation of modeling tools is built with web technologies and offers much more flexibility when it comes to their user experience, accessibility, reuse, and deployment options. One of the technologies behind this new generation of tools is the Graphical Language Server Platform (GLSP), an open-source client-server framework hosted under the Eclipse foundation, which allows tool providers to build modern diagram editors for modeling tools that run in the browser or can be easily integrated into IDEs such as Eclipse, VS Code, or Eclipse Theia. In this paper, we describe our vision of more flexible modeling tools which is based on our experiences from developing several GLSP-based modeling tools. With that, we aim at sparking a new line of research and innovation in the modeling community for modeling tool development practices and to explore opportunities, advantages, or limitations of web-based modeling tools, as well as bridge the gap between scientific tool prototypes and industrial tools being used in practice.

==> unblinded-ref.tex <==
% @article{Bork.20,
%   author       = {Dominik Bork and
%                   Steven Alter},
%   title        = {Satisfying Four Requirements for More Flexible Modeling Methods: Theory
%                   and Test Case},
%   journal      = {Enterp. Model. Inf. Syst. Archit. Int. J. Concept. Model.},
%   volume       = {15},
%   pages        = {3:1--3:25},
%   year         = {2020},
%   url          = {https://doi.org/10.18417/emisa.15.3},
%   doi          = {10.18417/emisa.15.3},
%   timestamp    = {Tue, 19 Jan 2021 16:13:51 +0100},
%   biburl       = {https://dblp.org/rec/journals/emisaij/BorkA20.bib},
%   bibsource    = {dblp computer science bibliography, https://dblp.org}
% }

@inproceedings{DeCarlo.22-er,
  author    = {Giuliano De Carlo and
               Philip Langer and
               Dominik Bork},
  editor    = {Jolita Ralyt{\'{e}} and
               Sharma Chakravarthy and
               Mukesh K. Mohania and
               Manfred A. Jeusfeld and
               Kamalakar Karlapalem},
  title     = {Rethinking Model Representation - {A} Taxonomy of Advanced Information
               Visualization in Conceptual Modeling},
  booktitle = {Conceptual Modeling - 41st International Conference, {ER} 2022, Hyderabad, India, 2022, Proceedings},
  series    = {Lecture Notes in Computer Science},
  volume    = {13607},
  pages     = {35--51},
  publisher = {Springer},
  year      = {2022},
  doi       = {10.1007/978-3-031-17995-2\_3}
}

@inproceedings{DeCarlo.22-models,
  author    = {Giuliano De Carlo and
               Philip Langer and
               Dominik Bork},
  editor    = {Eugene Syriani and
               Houari A. Sahraoui and
               Nelly Bencomo and
               Manuel Wimmer},
  title     = {Advanced visualization and interaction in GLSP-based web modeling:
               realizing semantic zoom and off-screen elements},
  booktitle = {Proceedings of the 25th International Conference on Model Driven Engineering Languages and Systems, {MODELS} 2022, Montreal, Quebec, Canada, 2022},
  pages     = {221--231},
  publisher = {{ACM}},
  year      = {2022},
  doi       = {10.1145/3550355.3552412}
}

@inproceedings{Glaser.21,
  author       = {Philipp{-}Lorenz Glaser and
                  Dominik Bork},
  title        = {The bigER Tool - Hybrid Textual and Graphical Modeling of Entity Relationships in {VS} Code},
  booktitle    = {25th International Enterprise Distributed Object Computing Workshop,
                  {EDOC} Workshop 2021, Gold Coast, Australia, October 25-29, 2021},
  pages        = {337--340},
  publisher    = {{IEEE}},
  year         = {2021},
  doi          = {10.1109/EDOCW52865.2021.00066}
}
